PipeTune: Pipeline Parallelism of Hyper and System Parameters Tuning for Deep Learning Clusters

DNN learning jobs are common in today's clusters due to the advances in AI driven services such as machine translation and image recognition. The most critical phase of these jobs for model performance and learning cost is the tuning of hyperparameters. Existing approaches make use of techniques such as early stopping criteria to reduce the tuning impact on learning cost. However, these strategies do not consider the impact that certain hyperparameters and systems parameters have on training time. This paper presents PipeTune, a framework for DNN learning jobs that addresses the trade-offs between these two types of parameters. PipeTune takes advantage of the high parallelism and recurring characteristics of such jobs to minimize the learning cost via a pipelined simultaneous tuning of both hyper and system parameters. Our experimental evaluation using three different types of workloads indicates that PipeTune achieves up to 22.6% reduction and 1.7x speed up on tuning and training time, respectively. PipeTune not only improves performance but also lowers energy consumption up to 29%.

==> problem.tex <==
%!TEX root = paper.tex




% Again soluton: An alternative to this would be to define the metric of interest as a weighted average between two or more useful metrics, and have the tuning process optimize towards that objective metric.

%% isabelly: this goes already towards solution

%We propose \sys, a framework for DNN training jobs that addresses the trade-offs between the impacts of certain hyperparameters on the system and the impacts of system parameters on the algorithms performance. \sys adopts a hybrid approach solution that covers both types of jobs mentioned earlier.

%For jobs type (i) we propose an offline approach that integrates the system parameters to the list of parameters to be tuned and relies on existing search algorithms to find the optimal values. As the characteristic of this job type allows it, later jobs can then take advantage of the found results and directly make use of an optimal configuration setup.

%However, the same strategy cannot be applied for jobs type~(ii). Therefore, we propose an alternative online approach that uses pipeline parallelism to enable faster training by tuning the systems parameters while hyperparameters are being tuned. The idea is to perform an exhaustive search for the system parameters having the epoch turnaround as granularity. This allows us to find the optimal configuration for a given setup within the first epochs. Once this configurations are know they are applied to the remaining iterations until a new setup comes and the same process is repeated.

%In the first case, the jobs consisting of unseen models present longer run times due to the added overhead of tuning the systems parameters for it. However, all other jobs take full benefit of the approach showing reduced run times. For the second cases, all jobs benefit from the approach in a linear manner. With that our hybrid approach can minimize average job time and makespan.


%--System scenarios (ideal): There is a deep neural networks cluster consisting of $N$ cores and each of cores has $Y$ memory. There is a queue that dispatches the job. There are two types workload scenarios: (i) training DNNs (same network) for different data sets, e.g., Google AD index, (ii) training different DNN on the same set of data. How the training jobs arrive?  What are the decisions to make? What assumptions we have? Assumption 1: we are given the privilege to do parameter turnings.  Assumption: jobs arrive and leave us to get the best accuracy

%-- What is wrong about the current setup? Where the challenges? It's very difficult questions. Related work only provides the partial solutions.

%--Objective: What do we want to achieve: the accuracy over energy ratio is optimized by tuning the parameters? 

%--Possible solution sketch:  What is the novelty? In contrast to the related work-- overlooking the system impacts of certain hyper parameters and the impact of system parameters on the algorithms performance

%Possible experiments: 

%\begin{itemize}
%    \item approach with known setup values is still better than pipe lined approach (to justify the need of a hybrid approach)
%    \item overhead of training for unseen model of job type (i)
%    \item makespan compared to baseline
%    \item average job completion time
%    \item energy
%\end{itemize}
 
